Search-based Crash Reproduction using Behavioral Model Seeding

Search-based crash reproduction approaches assist developers during debugging by generating a test case which reproduces a crash given its stack trace. One of the fundamental steps of this approach is creating objects needed to trigger the crash. One way to overcome this limitation is seeding: using information about the application during the search process. With seeding, the existing usages of classes can be used in the search process to produce realistic sequences of method calls which create the required objects. In this study, we introduce behavioral model seeding: a new seeding method which learns class usages from both the system under test and existing test cases. Learned usages are then synthesized in a behavioral model (state machine). Then, this model serves to guide the evolutionary process. To assess behavioral model-seeding, we evaluate it against test-seeding (the state-of-the-art technique for seeding realistic objects) and no-seeding (without seeding any class usage). For this evaluation, we use a benchmark of 124 hard-to-reproduce crashes stemming from six open-source projects. Our results indicate that behavioral model-seeding outperforms both test seeding and no-seeding by a minimum of 6% without any notable negative impact on efficiency.

==> Makefile <==
BASE_NAME = STVR-model-seeding
INPUTS    = $(wildcard *.tex) *.bib

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex $(INPUTS)
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(PDFLATEX) $< 
	$(PDFLATEX) $<

$(BASE_NAME).ps: $(BASE_NAME).tex 
	$(LATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(LATEX) $< 
	$(LATEX) $<
	
clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot 


==> sections/motivation.tex <==
\section{Motivations}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.77\textwidth]{figures/motivation/sample.png}
    \vspace{-1mm}
    \caption{Sample of the generated transition system for \texttt{java.util.Iterator}}
    \label{fig:motivation}
    \vspace{-3mm}
\end{figure*}
\pouria{I have added all of the hypothesis that we have about the reasons that model-seeding can perform better than other strategies to this section. However, I am not sure if this is the best place for this discussion. At this point in the paper, readers are not that much family about the previous studies. So, maybe this discussion confuses them here. Perhaps, adding it at the end of the background is more logical. we can change the name of the background section to background and motivations.}
The existing seeding techniques use only one resource to collect information for seeding. However, it is possible that the preferred resource does not have enough information about the usages of the interesting classes. For instance, test seeding only uses the carved call sequences from the execution of the existing test cases. If the existing test cases do not cover the behavior of the crash in the interesting classes, this seeding strategy may even misguide the search process. On the contrary, the behavioral model seeding collects the call sequences of each class from various resources and use all of them to infer a centralized transition system which represents the class usage. Since this strategy uses more resources compared to the other seeding strategies, it has a higher chance to seed a sequence which is closer to the crash reproducing scenario.

The improvement that we can achive Behavioral model seeding merges the observed call sequences to infer a transition system. This merging process may produce different sequences from the existing ones. For instance, Figure \ref{fig:motivation} demonstrates the generated transition system for java class \texttt{java.util.Iterator} from two call sequences: (\texttt{hasNext()}, \texttt{next()}) and (\texttt{hasNext()}, \texttt{next()},\texttt{hasNext()}, \texttt{next()}). This transition system contains a loop. So, the generated test from this mode can contain more than 2 method calls to the \texttt{next()} method.


If the number of observed call sequences is large, the seeding strategy needs a procedure to prioritize the call sequences for seeding. Seeding the random call sequences can misguide the search process. The existing seeding strategies do not have any procedure to fulfill this requirement. Behavioral model seeding uses the generated transition systems to define a technique for prioritizing the seeding candidates.


==> tables/crash-reproduction-ranking.tex <==
\begin{tabular}{ r l r l}
\textbf{Rank} & \textbf{Strategy} & \textbf{Rank value} & \textbf{Significantly better than} \\
\hline
1     & model s. 1.0    & 4.57    & (4), (5), (6), (7), (8), (9) \\
2    & model s. 0.2    & 4.63    & (4), (5), (6), (7), (8), (9) \\
3    & model s. 0.8    & 4.81    & (7), (8), (9) \\
4    & test s. 0.2        & 4.97    & (8), (9) \\
5    & no s.                 & 5.05    & \\
6    & model s. 0.5    & 5.05    & \\
7    & test s. 0.8        & 5.26    & \\
8    & test s. 0.5        & 5.32    & \\
9    & test s. 1.0        & 5.33    & \\
\end{tabular}

==> tables/fitness-evaluation-ranking.tex <==
\begin{tabular}{r l r l}
\textbf{Rank} & \textbf{Strategy} & \textbf{Rank value} & \textbf{Significantly better than} \\
\hline
1 & test s. 0.2		& 5.83 & (4), (5), (6), (7), (8), (9) \\
2 & no\_seeding		& 5.59 & (7), (8), (9) \\
3 & model s. 0.2	& 5.29 & (7), (8), (9) \\
4 & model s. 0.8	& 5.21 & (8), (9) \\
5 & model s. 1.0	& 5.18 & (8), (9) \\
6 & model s. 0.5	& 5.09 & (8), (9) \\
7 & test s. 0.5		& 4.73 & (8), (9) \\
8 & test s. 0.8		& 4.10 & \\
9 & test s. 1.0		& 3.98 & \\
\end{tabular}

==> tables/results.tex <==
\begin{tabular}{r l | r r r r r | r}
  \hline
\textbf{} & \textbf{} & \textbf{JFreeChart} & \textbf{Lang} & \textbf{Math} & \textbf{Mockito} & \textbf{XWiki} & \textbf{Total} \\ 
  \hline
    \multirow{6}{*}{\begin{sideways} no. s. \end{sideways}}
& $\overline{rep.}$ & 6.83 & 4.53 & 4.26 & 0.62 & 1.44 & 1.86 \\ 
& $\sigma_{r}$ & 3.71 & 5.00 & 4.80 & 2.50 & 3.45 & 3.79 \\ 
& $\overline{start}$ & 10.00 & 5.88 & 6.30 & 8.88 & 7.82 & 7.70 \\ 
& $\sigma_{s}$ & 0.00 & 5.07 & 4.37 & 3.07 & 4.04 & 4.09 \\ 
& $\overline{time}$ & 21364.90 & 34280.31 & 36976.26 & 58435.56 & 53496.58 & 50970.96 \\ 
& $\sigma_{t}$ & 28402.10 & 30931.20 & 30117.87 & 15122.68 & 21590.78 & 23859.99 \\ 
\hline
	\multirow{6}{*}{\begin{sideways}test s. 0.2 \end{sideways}}

& $\overline{rep.}$ & 4.17 & 4.35 & 4.52 & 1.25 & 1.45 & 1.86 \\ 
& $\sigma_{r}$ & 4.75 & 4.96 & 4.89 & 3.42 & 3.48 & 3.83 \\ 
& $\overline{start}$ & 5.00 & 5.88 & 6.37 & 8.94 & 7.84 & 7.63 \\ 
& $\sigma_{s}$ & 5.48 & 5.07 & 4.32 & 2.95 & 3.98 & 4.09 \\ 
& $\overline{time}$ & 36588.68 & 35312.98 & 35835.17 & 54537.51 & 53394.57 & 50932.92 \\ 
& $\sigma_{t}$ & 30716.15 & 30864.14 & 30014.25 & 20676.41 & 21749.06 & 23929.42 \\ 

\hline
	\multirow{6}{*}{\begin{sideways}test s. 0.5 \end{sideways}}
	
& $\overline{rep.}$ & 3.50 & 4.53 & 4.37 & 1.25 & 1.42 & 1.83 \\ 
& $\sigma_{r}$ & 4.46 & 5.00 & 4.94 & 3.42 & 3.44 & 3.79 \\ 
& $\overline{start}$ & 5.00 & 5.88 & 6.48 & 9.12 & 7.86 & 7.67 \\ 
& $\sigma_{s}$ & 5.48 & 5.07 & 4.53 & 2.42 & 4.00 & 4.11 \\ 
& $\overline{time}$ & 40719.33 & 34266.09 & 36012.86 & 54537.43 & 53565.42 & 51105.22 \\ 
& $\sigma_{t}$ & 29704.53 & 30943.45 & 30176.29 & 20676.64 & 21547.84 & 23783.81 \\ 

\hline
\multirow{6}{*}{\begin{sideways}test s. 0.8\end{sideways}}
& $\overline{rep.}$ & 3.17 & 4.65 & 4.41 & 1.25 & 1.41 & 1.82 \\ 
& $\sigma_{r}$ & 4.02 & 5.09 & 4.87 & 3.42 & 3.40 & 3.76 \\ 
& $\overline{start}$ & 5.00 & 5.88 & 6.30 & 9.00 & 7.88 & 7.66 \\ 
& $\sigma_{s}$ & 5.48 & 5.07 & 4.42 & 2.73 & 3.97 & 4.09 \\ 
& $\overline{time}$ & 43155.55 & 33559.11 & 35531.15 & 54538.21 & 53648.23 & 51142.84 \\ 
& $\sigma_{t}$ &  28476.33 & 30977.71 & 30341.39 & 20674.57 & 21469.61 & 23758.92 \\ 

\hline
\multirow{6}{*}{\begin{sideways}test s. 1.0\end{sideways}}

& $\overline{rep.}$ & 3.00 & 4.53 & 4.41 & 1.25 & 1.39 & 1.79 \\ 
& $\sigma_{r}$ & 3.95 & 5.00 & 4.92 & 3.42 & 3.40 & 3.76 \\ 
& $\overline{start}$ & 5.00 & 7.06 & 6.22 & 8.81 & 7.96 & 7.77 \\ 
& $\sigma_{s}$ & 5.48 & 4.70 & 4.52 & 3.06 & 3.93 & 4.04 \\ 
& $\overline{time}$ & 43789.27 & 34220.95 & 35802.61 & 54543.19 & 53790.68 & 51322.50 \\ 
& $\sigma_{t}$ &  28558.75 & 30983.57 & 30293.68 & 20661.35 & 21307.59 & 23608.38 \\ 

\hline
\multirow{6}{*}{\begin{sideways}model s. 0.2 \end{sideways}}

& $\overline{rep.}$ & 8.17 & 5.53 & 4.41 & 0.62 & 1.50 & 1.99 \\ 
& $\sigma_{r}$ & 2.48 & 4.87 & 4.92 & 2.50 & 3.42 & 3.84 \\ 
& $\overline{start}$ &  10.00 & 5.88 & 6.30 & 8.62 & 8.18 & 7.98 \\ 
& $\sigma_{s}$ &  0.00 & 5.07 & 4.44 & 3.05 & 3.74 & 3.87 \\ 
& $\overline{time}$ &  13554.63 & 29769.76 & 36213.37 & 58433.62 & 53157.38 & 50284.80 \\ 
& $\sigma_{t}$ &  24057.01 & 30278.29 & 30061.66 & 15130.21 & 21899.38 & 24317.44 \\ 

\hline
\multirow{6}{*}{\begin{sideways}model s. 0.5 \end{sideways}}
& $\overline{rep.}$ & 8.00 & 5.47 & 4.41 & 0.62 & 1.47 & 1.97 \\ 
& $\sigma_{r}$ & 2.76 & 4.82 & 4.80 & 2.50 & 3.41 & 3.81 \\ 
& $\overline{start}$ & 10.00 & 5.82 & 6.30 & 9.00 & 8.19 & 8.00 \\ 
& $\sigma_{s}$ & 0.00 & 5.03 & 4.33 & 2.39 & 3.73 & 3.83 \\ 
& $\overline{time}$ & 14553.18 & 29613.55 & 35928.44 & 58435.54 & 53311.63 & 50397.72 \\ 
& $\sigma_{t}$ &  24669.67 & 30290.77 & 30226.42 & 15122.78 & 21757.50 & 24249.20 \\ 

\hline
\multirow{6}{*}{\begin{sideways}model s. 0.8 \end{sideways}}

& $\overline{rep.}$ &  8.00 & 5.41 & 4.44 & 0.62 & 1.50 & 1.99 \\ 
& $\sigma_{r}$ &  3.16 & 4.89 & 4.85 & 2.50 & 3.45 & 3.85 \\ 
& $\overline{start}$ & 10.00 & 5.88 & 6.33 & 9.06 & 8.18 & 8.00 \\ 
& $\sigma_{s}$ & 0.00 & 5.07 & 4.40 & 2.26 & 3.71 & 3.82 \\ 
& $\overline{time}$ & 14105.00 & 31082.31 & 35555.19 & 58433.73 & 53134.76 & 50288.79 \\ 
& $\sigma_{t}$ & 24977.72 & 30207.12 & 30282.58 & 15129.79 & 21930.64 & 24334.44 \\ 

\hline
\multirow{6}{*}{\begin{sideways}model s. 1.0 \end{sideways}}

& $\overline{rep.}$ & 7.33 & 5.47 & 4.41 & 0.62 & 1.54 & 2.01 \\ 
& $\sigma_{r}$ & 3.44 & 4.87 & 4.92 & 2.50 & 3.46 & 3.85 \\ 
& $\overline{start}$ & 10.00 & 5.88 & 6.44 & 9.19 & 8.14 & 7.98 \\ 
& $\sigma_{s}$ & 0.00 & 5.07 & 4.39 & 2.29 & 3.77 & 3.86 \\ 
& $\overline{time}$ & 17610.62 & 29131.58 & 36090.69 & 58436.21 & 52981.30 & 50170.94 \\ 
& $\sigma_{t}$ & 27364.71 & 30625.43 & 29987.30 & 15120.17 & 22033.41 & 24404.40 \\ 
   \hline
\end{tabular}

==> tables/start-searching-ranking.tex <==
\begin{tabular}{r l r l}
\textbf{Rank} & \textbf{Strategy} & \textbf{Rank value} & \textbf{Significantly better than} \\
\hline
1 & model s. 1.0    & 4.91  & (4), (5), (6), (7), (8), (9) \\
2 & model s. 0.5   & 4.96 & (8), (9) \\
3 & test s. 1.0       & 4.96  & (8), (9) \\
4 &  test s. 0.5     & 4.98  & (8), (9) \\
5 & model s. 0.2  & 4.99  & (8), (9) \\
6 & model s. 0.8  & 5.00  & (8), (9) \\
7 & test s. 0.8      & 5.01   & (9) \\
8 & no\_seeding  & 5.06   & (9) \\
9 & test s. 0.2     & 5.14    &    \\
\end{tabular}
